Hidden Degrees of Freedom in Implicit Vortex Filaments

This paper presents a new representation of curve dynamics, with applications to vortex filaments in fluid dynamics. Instead of representing these filaments with explicit curve geometry and Lagrangian equations of motion, we represent curves implicitly with a new co-dimensional 2 level set description. Our implicit representation admits several redundant mathematical degrees of freedom in both the configuration and the dynamics of the curves, which can be tailored specifically to improve numerical robustness, in contrast to naive approaches for implicit curve dynamics that suffer from overwhelming numerical stability problems. Furthermore, we note how these hidden degrees of freedom perfectly map to a Clebsch representation in fluid dynamics. Motivated by these observations, we introduce untwisted level set functions and non-swirling dynamics which successfully regularize sources of numerical instability, particularly in the twisting modes around curve filaments. A consequence is a novel simulation method which produces stable dynamics for large numbers of interacting vortex filaments and effortlessly handles topological changes and re-connection events.

==> mathOfClebschVariables.tex <==
\section{Symplectic structure of our Clebsch variables}
In this section, we explain that our level function can be seen as a Clebsch variable, and it is the implicit counterpart of the celebrated \textit{Marseden--Weinstein} form for explicitly represented curves. We do so using the language of geometric mechanics \(\sim\) symplectic geometry. As for introductions to the subjects for interested readers, we refer to [Arnold "Mathematical methods of classical mechancis", Holm et al. "Geometric Mechanics and Symmetry: From Finite to Infinite Dimensions"].

As a preliminary, we briefly review Hamiltonian formulation of dynamics in geometric mechanics.  A hamiltonian dynamics is described by a triple \((M,\sigma, H)\) of some manifold \(M\), a non-degenerate 2-form \(\sigma\) on \(M\), and a function \(H\colon M\rightarrow \RR\) called a Hamiltonian. In particular, the pair \((M,\sigma)\) is called a symplectic structure or a symplectic manifold. There is a unique vector field \(X_H\) called the Hamiltonian vector field satisfying 
\begin{align}
    dH=\iota_{X_H} \sigma := \sigma(X_H,\cdot).
\end{align}
Then the time evolution of a state \(\bx\in M\) is simply given as an integral curve of \(X_H\) i.e. \(\dot{\bx}=X_H\). 
\begin{example}
    For a particle in \(\RR^n\) with generalized position \(\bq=(q_1,\ldots,q_n)\) and momentum \(\bp=(p_1,\ldots,p_n)\), a symplectic structure can be givem by  \(M=T\RR^n\) and \(\sigma=\sum_i dq_i \wedge dp_i\). Then, for a given Hamiltonian \(H\), the Hamiltonian vector field takes a well-known form \(X_H= \sum_i ^n \frac {\partial H}{\partial p_{i}} \frac {\partial }{\partial q_{i}} -\frac {\partial H}{\partial q^{i}} \frac {\partial }{\partial p_{i}} \). Setting a Hamiltonian  \(H(\bq,\bp)=\sum_i \frac{1}{2}p_i^2\)called the kinetic energy leads to the straight motion \(X_H=\sum p_i \frac{\partial}{\partial q^i}\).
\end{example}

We will now discuss the setting for the time evolutionary curves. We first see the case for explicitly represented curves \(\sF\), which is unlike the previous example, infinite dimensional as a curve contains infinite number of points.  In the seminal work of Marsden \& Weinstein [cite], they found a symplectic structure,
\begin{align}
    \sigma_{\rm MW} \in \Omega^2(\sF),\quad \sigma_{\rm MW}\big\vert_{\gamma}(\dot\gamma,\mathring\gamma) = \oint_{\bigsqcup_{i=1}^m\SS^1} \det(\dot\gamma,\mathring\gamma,d\gamma).
\end{align}
Thanks to this finding,  we can define a dynamics for curves by giving a Hamiltonian  \(H\colon \sF \rightarrow \RR\). In the case of vortex filaments, it is given as 
\begin{align}
    H(\gamma) = \iiint_{M}{1\over 2}|\bu_\gamma|^2\, dV.
\end{align}

We now study the case for our implicit representation as a Clebsch variable. Traditionally, a Clebsch map is given in the following way. Let \((\Sigma, \sigma)\) be a pair of a manifold and a fixed \(2\)-form on it. A map \(s:M\rightarrow\Sigma\) is called a Clebsch map for \(\alpha \in\Omega^2(M) \) if
 \(\alpha = s^* \sigma\). Then the pair of the space
\begin{align}
     \cM= \lbrace s\colon M \rightarrow \Sigma \rbrace
\end{align}
and \(\sigma_M\in \Omega^2(\cM)\) given by  
\begin{align}
     \sigma_\cM (\dot s ,\mathring s)=\int _M \sigma( \dot s ,\mathring s)
\end{align}
for \(\dot s ,\mathring s \in \lbrace M\rightarrow T\Sigma \rbrace\) defines a symplectic structure.

Our level functions can be seen as Clebsch variables by setting \(\Sigma=\CC \), \(\sigma=\delta_0\), and \(\alpha=\delta_\gamma\) for some \(\gamma \in \sF\). Note that the Dirac delta \(\delta_0\) is not a 2-form but a linear function on compactly supported smooth functions \(\Omega_c ^0(M)\).  We can, however, formally regard \(\delta_0 \in \Omega^2 (M)\) in the way that it is to be integrated over \(\CC \approx \RR^2\) by 
\begin{align}
\delta_0 (f) := f(0) \approx \int_\CC f\wedge \delta_0
\end{align}
for \(f \in \Omega^0_c(M) \).
Then the equivalence class of level functions we defined is also written as \(\psi_1 \sim \psi_2\) if \(\psi_1^* \delta_0 =  \psi_2^* \delta_0\).

Likewise the argument for general \(2\)-Clebsch maps, we have a symplectic form on the space \(\cM =  \tilde{\cM} / \sim\) given by
\begin{align}
     \sigma_\cM ([\dot \psi], [\mathring \psi] )
     &=\int _M \delta_0( \dot \psi  ,\mathring \psi )\\
     &=\int_M \psi^* i_{\dot \psi } \circ i_{\mathring \psi } \ \delta_0 \  dV\\
     &= \int_M i_{d\psi^{-1}(\dot \psi )} \circ i_{d\psi^{-1}(\mathring \psi )} \psi^* \delta_0 \ dV\\
     &=\int_M \delta_{\gamma} (\dot \gamma, \mathring \gamma) \ dV
\end{align}
where \(\gamma=\psi^{-1}(0)\) is the curve represented by \(\psi\), and \(\dot \gamma=d\psi^{-1}(\dot \psi )\) and \(\mathring \gamma= d\psi^{-1}(\mathring \psi ) \) are vector fields on \(\gamma\).


==> overview.tex <==
\section{Overview}
 
\cCW{We needed a buffer to transition from the related work to the next section. Without it, the transition is too sudden of a jump from high-level discussion to low-level details. If you don't like the extra section, I can try to cram in a transition at the start of \secref{sec:representation}, but I thought this way was more natural.}

We now begin our description of how we simulate implicit filament dynamics. \secref{sec:representation} discusses how to represent curves mathematically, revealing a number of redundant degrees of freedom. \secref{sec:untwisted} details how we can exploit these redundant degrees of freedom to create a more regular and numerically robust representation for both the geometry of filaments and their dynamics. \secref{sec:algorithms} and  \secref{sec:applications} describe our algorithm and results, and we conclude with a discussion in \secref{sec:conclusion}.

==> some_thoughts.tex <==
\section{Idea of our algorithm}
\cSI{This is just a rough sketch of ideas.}

Our setting in a broad sense is a level-set method with codimension 2.  This means that we express the time evolution of space curves by representing the curves as level-sets of some two functions and evolve these functions in time.

In order to model physical phenomena with this setting, we need to specify the functions and their time evolution. For example, quantum vortices appearing in the Bose-Einstein condenstates of superfluids are modeled as the singularities of the Gross-Pitaevski equation.

In the sequel, we will make a particular choice of the functions and their evolution law to relate our codimensional expression to the dynamics of (quantum) ideal fluids.

\subsection{Overview}
Our algorithm can be understood as an advection-projection scheme in a broad sense. This is done by leveraging the duality between different representation of the fluid state and the equivalence of the incompressible quantum Euler equation and the Schrodinger equation.

\subsection{Duality of different representations}
We use three representations of the fluid state. 
\begin{itemize}
     \item velocity field 
     \begin{align}
          \sV = \left\lbrace v\colon M\rightarrow \RR^3 \right\rbrace
     \end{align}
     \item wave function
     \begin{align}
          \varPsi=  \left\lbrace  \psi\colon M \rightarrow \CC^1 \right\rbrace
     \end{align}
     \item space curves
     \begin{align}
          \sF= \left\lbrace \gamma \colon\textstyle\bigsqcup_{i=1}^m\SS^1 \rightarrow M \cup \{\infty\}  \right\rbrace
     \end{align}
\end{itemize}
They can be translated to each other. From given space curves to a velocity field, we have the Biot-Savart law 
\begin{align}
     v_{\gamma}(x) :=\sum_{i} \frac{\Gamma_{i}}{4 \pi} \oint \gamma_{i}^{\prime}(s) \times \frac{x-\gamma_{i}(s)}{\left|x-\gamma_{i}(s)\right|^{3}} d s
\end{align}
where $\{\Gamma_i\}_i$ are real values called the strengths of the filaments. A wave function \( \psi (x):= \rho(x) e^{i \theta (x)}\) can be converted to a velocity field by
\begin{align}
     v_\psi(x):=\nabla \theta(x).
\end{align}
We can see that velocitiy fields created from \(\psi\) are quantized in the way that circulation of \(v_\psi\) along any closed curve is \(2\pi k\) with some integer \(k\). Note also that the incompressibility condition \(\rho(x)\equiv 1\), this gives an injection from wave functions to velocity fields up to constant phase shift in \(\psi\). Then these two relations give us the correspondance between wave functions and space curves by
\begin{align}
     v_\gamma=v_\psi.
\end{align}
We see that these maps between three representations are not bijective i.e. both \( \{ v_\gamma\}_\gamma\) and \( \{ v_\psi \}_\psi\) are just subsets of \(\sV\) and \( \{ v_\gamma\}_\gamma\) is a subset of  \( \{ v_\psi\}_\psi\) \cSI{This part is important when we talk about {\it projection} later}.

We also have a duality between the Schrodinger equation and the Euler equation for fluid mechanics. 

\subsection{Equivalence of two equations}
Through Madelung transformation
\begin{align}
     (m, \theta) \rightarrow \psi:=\sqrt{m} e^{i\theta},
\end{align}
the Schr\"odinger equation with the potential term
\begin{align}
     i\hbar \partial_t \psi =\left[{\frac {-\hbar ^{2}}{2m}}\Delta+V \right]\psi 
\end{align}
is equivalent to the (quantum) Euler equation,
\begin{align}
      \partial _{t}\mathbf {u} = -\nabla_\mathbf{u}  \mathbf {u} -{\frac {1}{m}}\mathbf {\nabla }P
\end{align}
with \(\mathbf {u} =\frac{1}{m} \nabla \theta \). The additional assumption of incompressibility \(m=1\) leads to the incompressible Schr\"odinger equation and quantum Euler equation.

\subsection{Time evolution of level-functions}
A typical numerical computation of the dynamics of ideal fluids is performing two operations called advection and projection \TODO{cite Stable Fluids}. Our proposed algorithm is understood as an advection - projection scheme in a broad sense. First, the directional derivative \( \nabla_u u\) in the Euler equation is known to convect the current state of the velocity field \(u\) along itself. The term \( \Delta \psi\) in the Schr\"odinger equation can be also seen as advection in the way that it transports the current state \(\psi\). 

Second, physically, projection is performing the computation of the pressure term. But mathematically, projection is indeed to project the current state of \(u\) or \(\psi\) to the space of certain canonical states. In the case of the incompressible Euler equation, this space consists of the divergence-free velocity fields. For the incompressible Schr\"odinger equation, this space is the collection of the wave functions satisfying 
\begin{align}
     \langle\Delta \psi, i \psi\rangle_{\mathbb{R}}=0 \quad \textup { and } \quad|\psi|^{2}=1.
\end{align}
As we saw, there are operations for both equations that correspond to advection and projection for velocity fields and wave functions respectively. And as far as we can travel between the space of the velocity fields and the wave functions, we could perform advection and projection to either of them.

In our case, we will advect \(\psi\) along \(v_\psi\) and perform projection of \(\psi\) onto the space of the Biot-Savart wave functions i.e. there exist curves \(\gamma\) s.t. \(v_\psi = v_\gamma \). Actually, we could replace the advection part by  computation of \(\Delta \psi\) in Schrodinger's smoke fashion. \cSI{I think we should include an experiment comparing our standard advection and Schrodinger's smoke advection}.

\cSI{Probably, we should  explain already here a direct computation of the incompressible quantum Euler equation / Schrodinger equation is challenging due to finite state machine problem caused by classical pressure projection in a discrete setting. We can say that our projection can work at sub-grid level.}

\subsection{Choices of the level functions}
As we saw, the wave function \(\psi = e^{i \theta}\) reads the incompressible Schr\"odinger equation (equivalently the incompressible quantum Euler equation). In that case, a spatial curve with \(v_\gamma = \nabla \theta\) is given as the singularities of \(\psi\). A smooth wave function yielding the same velocity field is
\begin{align}
     \psi(x) = \textup{dist}(\gamma,x) e^{i \theta} 
\end{align}

The either of the above choices makes the system the incompressible quantum Euler equation / incompressible Schrodinger equation and allows us to blend each term of them as we did.

\subsection{Solid angle computation}
A typical computation is to sum up the areas of all the spherical triangles \( ( Z,p_i,p_{i+1} )\) with some fixed pole $Z$. This have some issue... Ours stems from the Hopf fibration...

\subsection{Obstacles}
\paragraph{Pressure projection}
We can modify the Biot-Savart velocity field by adding the gradient of a scalar function. Kelvin transform, Weissmann\&Pinkall, or perform classical pressure projection to the velocity field stored on the grids.

\paragraph{Quantum potentials}

\section{Applications}
\subsection{(Quantum) vortex filaments}
Physically (quantum) vortex filaments are topological defects appearing in (super)fluids.

Mathematically they are Dirac-delta type weak solutions to incompressible quantum Euler equation / \(\CC\)-valued incompressible Schrodinger equation whose support are space curves. 

To the best of our knowledge, our method is the first numerical scheme for this equation (though it is limited to a certain class of weak solutions i.e. filaments) as this equation holds a fundamental challenge for discretization. 

\paragraph{Why numerics of quantum incompressible Euler equation is challenging}
Quantization (ultradiscretization) of vorticity resulting in finite state machine...

Practically, happening due to classical pressure projection.
something
\subsection{Smoke simulation}
We can simulate smoke using the Biot-Savart velocity field generated from filaments.



